Nonlinear Model Predictive Control with Enhanced Actuator Model for Multi-Rotor Aerial Vehicles with Generic Designs

In this paper, we propose, discuss, and validate an online Nonlinear Model Predictive Control (NMPC) method for multi-rotor aerial systems with arbitrarily positioned and oriented rotors which simultaneously addresses the local reference trajectory planning and tracking problems. This work brings into question some common modeling and control design choices that are typically adopted to guarantee robustness and reliability but which may severely limit the attainable performance. Unlike most of state of the art works, the proposed method takes advantages of a unified nonlinear model which aims to describe the whole robot dynamics by explicitly including a realistic physical description of the actuator dynamics and limitations. As a matter of fact, our solution does not resort to common simplifications such as: 1) linear model approximation, 2) cascaded control paradigm used to decouple the translational and the rotational dynamics of the rigid body, 3) use of low-level reactive trackers for the stabilization of the internal loop, and 4) unconstrained optimization resolution or use of fictitious constraints. More in detail, we consider as control inputs the derivatives of the propeller forces and propose a novel method to suitably identify the actuator limitations by leveraging experimental data. Differently from previous approaches, the constraints of the optimization problem are defined only by the real physics of the actuators, avoiding conservative -- and often not physical -- input/state saturations which are present, e.g., in cascaded approaches. The control algorithm is implemented using a state-of-the-art Real Time Iteration (RTI) scheme with partial sensitivity update method. CONTINUES...

==> figures/tikz/ident_procedure.tex <==
%\documentclass[./../main.tex]{subfiles}

\begin{document}
\tikzset{
%font={\tiny},%{\fontsize{4pt}{6}\selectfont},
  block/.style  = {draw, fill=yellow!10, thick, rectangle, text centered,
  	 rounded corners, minimum height = 1.5em, text width=14em,
  	 minimum width = 10em, inner sep = .2em, node distance=2.5em and 1.5em},
  block_terminal/.style  = {draw, fill=yellow!10, thick, rectangle, double, double distance=0.1em, text 	
  	 centered,rounded corners, minimum height = 1.5em, text width=14em,
  	 minimum width = 10em, inner sep = .4em, node distance=2.5em and 1.5em},
  decision/.style = {draw, fill=red!20!white, diamond,
  	 text width=8em, text badly centered, aspect=2, inner sep=-5pt},
  mytext/.style = {text centered, rounded corners, minimum height = 2.2em,
  	 text width=12em, minimum width = 6em, inner sep = .2em, 
  	 node distance=1em and 1em},
  condition/.style = {fill=cyan!10!white, rectangle, rounded corners, inner sep = .2em, yshift=.3em},
  line/.style={draw, -stealth, thick, black}   
}
\resizebox {\columnwidth} {!} {

\begin{tikzpicture}[remember picture]
	\node[block_terminal] (S1) {select different set-points $\doubleu_h^*$, $\ h \in [1,H]$, that span $[\underline{\doubleu},\overline{\doubleu}]$};
	\node[block, below =of S1] (S1bis) {generate a sequence of ramps with increasing slopes, centered at $\doubleu_h^*$};
	\draw[line] (S1) -- node [condition] {controlling the motor in velocity}(S1bis);
	\node[block, below =of S1bis] (S2) {compute $e_{\doubleu}$ at the set-point $\doubleu_h^*$};
	\draw[line] (S1bis) -- node [condition] {using $e_{\doubleu}=\doubleu_d-\doubleu$}(S2);
	\node[block, below =of S2] (S3) {compute $e_{f}$ at the set-point $\doubleu_h^*$};
	\draw[line] (S2) -- node [condition] {using eq.~\eqref{eq:e_f}} (S3);
	\node[block, below =of S3] (S3bis) {estimate $\underline{\dot{\doubleu}},\overline{\dot{\doubleu}}$ at the set-point $\doubleu_h^*$};
	\draw[line] (S3) -- node [condition] {by visual inspection} (S3bis);	
	\node[decision, below=of S3bis] (D1) {is $h > H$ ?};
	\draw[line] (S3bis) -- node [condition] {$h\leftarrow h+1$}(D1);
	\node[block, below =of D1] (S4) {estimate $\underline{\dot{\doubleu}},\overline{\dot{\doubleu}}$ as a function of $\doubleu$};
	\draw[line] (D1) -- node [near start,xshift=1.8em,yshift=0.7em] {yes} node [condition] {interpolating between H points}(S4);
	\node[block_terminal, node distance=2.5em and 1.5em, below =of S4] (S5) {estimate $\underline{\dot{f}},\overline{\dot{f}}$ as a function of $f$};
	\draw[line] (S4) -- node [condition] {using eq.s~\eqref{eq:f_i} \& \eqref{eq:dot_f_i}} (S5);
	%\node [mycircle, below =of S5] (exit) {.};
	%\node[draw, circle, ultra thick,minimum size=1.5em ] (exit_bis) at (exit) {};
	%\draw[line] (S5) -- (exit_bis);
	\coordinate (pathback1) at ($(D1.west)$);
	\coordinate (pathback2) at ($(D1.west)+(-1.8,0em)$);
	\draw[line] (pathback1) -- node [near start,yshift=0.5em] {no} (pathback2) 
		node [condition, yshift=9em, rotate=-90] {repeating}
		|- ($(S1bis.west)$);
	
\node[block_terminal,text width=10em, node distance=2.5em and 2.5em, left =of S1, xshift=0.4em, yshift=-0.6em] (SS1) {collect information about motor/controller safety constraints};
\node[block,text width=10em, node distance=2.5em and 2.5em, left =of S4] (SS2) {estimate $\underline{\doubleu},\overline{\doubleu}$};
\draw[line] (SS1) -- node [condition, rotate=-90] {combining such limits}(SS2);
\node[block_terminal, node distance=2.5em and 2.5em, text width=10em, below =of SS2,yshift=-0.1em] (SS3) {estimate $\underline{f},\overline{f}$};
\draw[line] (SS2) -- node [condition] {using eq.~\eqref{eq:f_i}}(SS3);

%\node[above =of SS1, node distance=0.5em and 2em] (state_node) {State constraints};
\end{tikzpicture}

 } % resizebox

\end{document}


==> tables/contributions.tex <==
%%%\begin{center}
\begin{table*}[htp]
%%%\begin{table*}[h]
\caption{Condensed illustration of the presented works on MPC in the recent literature of aerial robotics.
%%%\captionsetup{margin=0.2in} % further reduce the lateral margins for the caption
%%%\vspace{0.5em} \newline 
%%%Legend: l = linear, 
%%%nl = nonlinear, 
%%%e = explicit, 
%%%h = hybrid,
%%%ad = axes-decoupled, 
%%%lqr = linear quadratic regulator, 
%%%sim = simulations, 
%%%exp = experiments,  
%%%r = trajectory regulation, 
%%%t = trajectory tracking, 
%%%p.c. = position control,
%%%a.c. = attitude control,
%%%f.c. = force control, 
%%%ps.c. = partial-state control, 
%%%fs.c. = full-state control,
%%%t.p. = trajectory planning, 
%%%on = onboard, 
%%%off = offboard, 
%%%%n.s. = not specified, 
%%%m.b. = move block technique, 
%%%h.l. =  prediction horizon length, 
%%%N = prediction horizon steps, \newline
%%%d.h. = diminishing horizon.
}
%%%%%
	%%%\vspace{0.5em}
	\centering
	\begin{minipage}{\textwidth}
	\centering
	{\footnotesize
	\begin{tabular}{|g|c|}
		\hline
%%%		\rule{0pt}{12.5pt}
%%%		{\textbf{Symbol}}  & {\textbf{Description}} \\[5pt]
		{\textbf{Symbol}}  & {\textbf{Description}} \\
		\hline
		\multicolumn{2}{ |c|}{\emph{Problem Formulation}} \\
		\hline
		l & linear \\
		nl & nonlinear \\
		lqr & linear quadratic regulator \\ 
		h & hybrid \\
		ad & axes-decoupled \\
%%%		h & hybrid \\
%%%		ad & axes-decoupled \\
		\hline           
	\end{tabular}
	\renewcommand\arraystretch{1.167}
	\begin{tabular}{|g|c|}
		\hline
		\multicolumn{2}{ |c|}{\emph{Problem Resolution}} \\
		\hline
		i & implicit \\
		e & explicit \\
		\hline
		\multicolumn{2}{ |c|}{\emph{Validation}} \\
		\hline
		sim & simulations \\
		exp & experiments \\
%%%		r & trajectory regulation \\ 
%%%		t & trajectory tracking \\
		\hline
	\end{tabular}
	\renewcommand\arraystretch{1}
	\begin{tabular}{|g|c|}
		\hline
		\multicolumn{2}{ |c|}{\emph{Problem targeted}} \\
		\hline
		p.c. & position control \\
		a.c. & attitude control \\
		f.c. & force control \\
		ps.c. & partial-state control \\ 
		fs.c. & full-state control \\
		t.p. & trajectory planning \\
		\hline
	\end{tabular}
	\renewcommand\arraystretch{0.857}
	\begin{tabular}{|g|c|}
		\hline
		\multicolumn{2}{ |c|}{\emph{Implementation details}} \\
		\hline
		on & on-board the vehicle\\
		off & off-board the vehicle \\ 
		m.b. & move block technique \\ 
		$t_H$ &  prediction horizon length \\ 
		$N$ & prediction horizon steps \\
		d.h. & diminishing horizon \\ 
		$T_{\text{MPC}}$ & sample time \\
		\hline
	\end{tabular}
	} % \small
	\end{minipage}
		
	\vspace{1em}
%%%%%
\renewcommand\arraystretch{1.3}
%%%\renewcommand\arraystretch{1.2}
\label{tab:contributions}
\resizebox{\textwidth}{!}{
%%%\begin{tabu} to 0.95\textwidth {|[1pt] c |[2pt] g | g | g | g |[1pt]}
\begin{tabu} to \textwidth {|[1pt] c |[2pt] g | g | g | g |[1pt]}
%
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}*{\textbf{MPC paper}} 
&\textbf{state 
\& input} 
& \textbf{l / nl / lqr}				
& \textbf{sim / exp}
& \textbf{platform} 	 
\\
%\cline{2-5}
& \textbf{cost function 
\& constraints} 
%%%& \textbf{r / t} 	
& \textbf{i / e} 	
& \textbf{use}  
& \textbf{horizon} 
\\
\tabucline[2pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{alexis2014robust} \citedb{alexis2016robust}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \phi \ \theta]^{\top}$ 
\& $\mathbf{u}=[\phi^r\,\theta^r\,T]^{\top}$
& l (ad)
& exp 
& quadrotor, tilting trirotor 	 
\\
%\cline{2-5}
& $\max_{w}\max_{j}||\mathbf{Cx}_{k+j|k}||_{\infty}$ 
\& $\mathbf{u}_{k+j|k}\in\mathcal{U}, \mathbf{x}_{k+j|k}\in\mathcal{X},\mathbf{w}_{k+j|k}\in\mathcal{W}$ 
%%%& t
& e
&  p.c. (on)	
& $t_H=0.48\si{s},0.6\si{s}$ / $N=6$ 
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{baca2016embedded}} 
& $\mathbf{x}_k=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \ddot{\mathbf{p}}^{\top} \, \ddot{\mathbf{p}}_u^{\top} \, \ddot{\mathbf{p}}_d^{\top}]^{\top}_{x,y}$ 
\& $\mathbf{u}_k=[\phi^r \, \theta^r]^{\top}$
& l (ad)
& exp 
& quadrotor%s	 
\\
%\cline{2-5}
&  $\frac{1}{2}\sum_{i=1}^{m-1}\big(\mathbf{e}^T_{x,i}\mathbf{Q}\mathbf{e}_{x,i} + \mathbf{u}^T_i\mathbf{R}\mathbf{u}_i\big) + \frac{1}{2}\mathbf{e}^T_m\mathbf{S}\mathbf{e}_m$ 
%\& $\mathbf{u}_{i}\in\mathcal{U}$
\& unconstrained
%%%& t
& e
&  p.c. (on)	
& $t_H=2.2\si{s}$ / $N=200$ (m.b.) 
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{baca2017autonomous}} 
& $\mathbf{x}_k=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \ddot{\mathbf{p}}^{\top} \, \ddot{\mathbf{p}}_u^{\top} \ , \ddot{\mathbf{p}}_d^{\top}]^{\top}_{x,y}$ 
\& $\mathbf{u}_k=[\phi^r \, \theta^r]^{\top}$
& l (ad)
& exp 
& hexarotor	 
\\
%\cline{2-5}
&  $\frac{1}{2}\sum_{i=1}^{m-1}\big(\mathbf{e}^T_{x,i}\mathbf{Q}\mathbf{e}_{x,i} + \mathbf{u}^T_i\mathbf{R}\mathbf{u}_i\big) + \frac{1}{2}\mathbf{e}^T_m\mathbf{S}\mathbf{e}_m$ 
%\& $\mathbf{u}_{i}\in\mathcal{U}$
\& $\mathbf{x}_i\in \mathcal{X},\mathbf{u}_{i}\in\mathcal{U}$
%%%& t
& i
&  t.p. (on)	
& $t_H=8\si{s}$ / $N=800$ (m.b.) 
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{BANGURA201411773}} 
& $\mathbf{x}=[{\mathbf{p}}^{\top} \, \dot{\mathbf{p}}^{\top} \, {F}]^{\top}$ 
\& $\mathbf{u}=[\boldsymbol{\omega}^{\top} \, \dot{T}]^{\top}$
& l
& exp 
& quadrotor	 
\\
%\cline{2-5}
&  $\sum_{i=0}^{N-1}\big(\mathbf{e}_{x,k+i|k}^T\mathbf{Q}\mathbf{e}_{x,k+i|k} + \mathbf{u}_{k+i|k}^T\mathbf{R}\mathbf{u}_{k+i|k}\big)$ 
\& unconstrained
%%%& t
& e
&  p.c. (on)	
%%%& h.l.=0.3125s / N=5 
& $t_H \approx 0.31\si{s}$ / $N=5$ 
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{bemporad2009hierarchical}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \boldsymbol{\Theta}^{\top} \,\dot{\boldsymbol{\Theta}}^{\top} \, \int{e_z}dt]^{\top}$ 
\& $\mathbf{u}=[\boldsymbol{\tau}^{\top} \, T]^{\top}$
& l / h
& sim 
& quadrotor	 
\\ 
%\cline{2-5}
&  $\sum_{i=0}^{N-1} \sum_{j=1}^{n_y} \big(\mathbf{e}_{x_j,i}^T\mathbf{Q}\mathbf{e}_{x_j,i} + \boldsymbol{\Delta}\uv_{x_j,i}^T\mathbf{R}\boldsymbol{\Delta}\uv_{x_j,i}\big)$ 
\& $\mathbf{u}\in\mathcal{U}, \mathbf{x}\in\mathcal{X}$
%%%& t
& i
&  {\scriptsize p.c. / t.p. (off)}
& $t_H \approx1.5\si{s}$ / $N=20$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{bouffard2012learning}} 
& $\mathbf{x}=[x_1\ , \dot{x}_1 \, \theta_1 \, \dot{\theta}_1 \, x_2 \, \dot{x}_2 \, \theta_1 \, \dot{\theta}_1 \, x_3 \, \dot{x}_3]^{\top}$ 
\& $\mathbf{u}=[\theta_1^r \, \theta_2^r \, T^r]^{\top}$
& l
& exp  
& quadrotor	(+ net) 
\\ 
%\cline{2-5}
&  $\sum_{j=0}^{N-1} \big( \mathbf{e}_{x,j}^T \mathbf{Q} \mathbf{e}_{x,j} +
\mathbf{e}_{u,j}^T \mathbf{R} \mathbf{e}_{u,j}  \big) + 
\mathbf{e}_{x,N}^T \mathbf{P} \mathbf{e}_{x,N}$ 
\& $\mathbf{u}\in\mathcal{U}, \mathbf{x}\in\mathcal{X}$
%%%& t
& i
&  p.c. (on)
& $t_H\approx0.38\si{s}$ / $N=15$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{darivianakis2014hybrid}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \phi \ \theta]^{\top}$ 
\& $\mathbf{u}=[\phi^r \, \theta^r \, T]^{\top}$
& l (ad)
& exp 
& quadrotor (+ writing tool)	 
\\ 
%\cline{2-5}
&  $\sum_{k=0}^{N-1} \big(\mathbf{e}^T_{x,k}\mathbf{Q}\mathbf{e}_{x,k} + \mathbf{u}^T_k\mathbf{R}\mathbf{u}_k\big) + \frac{1}{2}\mathbf{e}^T_N\mathbf{P}\mathbf{e}_N$ 
\& $\mathbf{x}_{k}\in \mathcal{X},\mathbf{u}_{k}\in\mathcal{U}$
%%%& t
& e
&  \scriptsize{p.c. / f.c. (on)}
& $t_H=0.2\si{s}$ / $N=10$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{falanga2018pampc}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \mathbf{q}^{\top}]^{\top}$ 
\& $\mathbf{u}=[\boldsymbol{\omega}^{\top} \, T]^{\top}$
& nl
& exp 
& quadrotor	 
\\ 
%\cline{2-5}
&  $\sum_{i=1}^{N}\big([\mathbf{e}^T_{x,i}, \mathbf{e}^T_{z,i}] diag(\mathbf{Q}_{x,i},\mathbf{Q}_{p,i}) [\mathbf{e}^T_{x,i} \mathbf{e}^T_{z,i}]^T \big)$
%+ \mathbf{e}^T_{x,N}\mathbf{Q}_{x,N}\mathbf{e}_{x,N}$ if you want to replace this, index of the sum up to N-1 
\& $\mathbf{x}\in \mathcal{X},\mathbf{u}\in\mathcal{U}$
%%%& t
& i
&  t.p. (on)
& $t_H=2\si{s}$ / $N=20$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{foehnonboard}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \mathbf{q}^{\top}]^{\top}$  
\& $\mathbf{u}=[\boldsymbol{\omega}^{\top} \, T]^{\top}$
& lqr
& exp 
& quadrotor	 
\\ 
%\cline{2-5}
&  $\int_0^{\infty}\mathbf{e}^T_{x}(t)\mathbf{Q}\mathbf{e}_{x}(t)+\mathbf{e}^T_{u}(t)\mathbf{R}\mathbf{e}_{u}(t)\ dt$
%%%\& lqr, so unconstrained
\& unconstrained
%%%& t
& e
&  p.c. (on)
& $t_H=\infty$ / $T_{\text{MPC}}=0.1\si{s}$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{geisert2016trajectory}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \boldsymbol{\Theta}^{\top} \, \dot{\mathbf{p}}^{\top} \,\boldsymbol{\omega}^{\top} \, \bar{w}_i|_{i=1}^4]^{\top}$
\& $\mathbf{u}=[\dot{\bar{w}}_i|_{i=1}^4]^{\top}$
& nl
& sim 
& quadrotor	(+ slung load) 
\\ 
%\cline{2-5}
&  $\sum_{i=1}^{N-1}\big(\mathbf{e}_{p,i}^T\mathbf{Q}\mathbf{e}_{p,i}\big) + \boldsymbol{\omega}^T_N C \boldsymbol{\omega}_N$
\& $\mathbf{u}\in\mathcal{U}$
%%%& t
& i
& fs.c. (off)
& $t_H=8\si{s}$ / $N=60$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{hofer2016application}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \boldsymbol{\Theta}^{\top} \, \dot{\mathbf{p}}^{\top} \,\boldsymbol{\omega}^{\top}]^{\top}$ 
\& $\mathbf{u}=[T_{y,i}|_{i=1}^3,T_z]^{\top}$
& l
& sim \& exp 
& ducted-fans + flaps 
\\ 
%\cline{2-5}
&  $\frac{1}{2}\int_0^{\infty}\mathbf{x}^T(t)\mathbf{Q}\mathbf{x}(t)+\mathbf{u}^T(t)\mathbf{R}\mathbf{u}(t)\ dt$
\& $\mathbf{u}\in\mathcal{U}$
%%%& t
& i
&  fs.c. (on)
& $t_H=\infty$ / $T_{\text{MPC}}=0.02\si{s}$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{kamel2015fast}} 
& $\mathbf{x}=[\{\mathbf{R}_B^W\}_{ij}, \boldsymbol{\omega}^{\top}]^{\top}$  
\& $\mathbf{u}=[{f_i}|_{i=1}^6]^{\top}$
& nl
& sim \& exp 
& hexarotor 
\\ 
%\cline{2-5}
&  $\int_t^{t+T_h}\mathbf{e}_x^T(t)\mathbf{Q}_x\mathbf{e}_x(t)+\mathbf{e}_u^T(t)\mathbf{Q}_u\mathbf{e}_u(t)dt$
%+\mathbf{u}^T(t)\mathbf{R}\mathbf{u}(t)\ dt$  
\& $\mathbf{x}\in \mathcal{X}, \mathbf{u}\in\mathcal{U}$
%%%& t
& i
& a.c. (on)
& $t_H=50\si{ms}$ / $N=10$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{kamel2017linear}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, _I\phi \, _I\theta]^{\top}$  
\& $\mathbf{u}=[_I\phi^r \, _I\theta^r \, T]^{\top}$
& l vs nl
& exp  
& hexarotor 
\\ 
%\cline{2-5}
&  $\sum_{i=1}^{N-1}\big(\mathbf{e}^T_{x,i}\mathbf{Q}\mathbf{e}_{x,i} + \mathbf{e}^T_{u,i}\mathbf{R}\mathbf{e}_{u,i}\big) + \mathbf{e}^T_{x,N}\mathbf{Q}\mathbf{e}_{x,N}$
\& $\mathbf{u}\in\mathcal{U}$
%%%& t
& i
& p.c. (on)
& $t_H=2\si{s}$ / $N=20$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{kocer2018centralized}} 
& $\mathbf{x}=[\mathbf{p}_W^{\top} \, \dot{\mathbf{p}}_B^{\top}]^{\top}$  
\& $\mathbf{u}=[\phi, \theta, \psi, F_z]$
& nl
& exp  
& quadrotor (close to ceiling)
\\ 
%\cline{2-5}
&  $\int_t^{t+N}\mathbf{e}_x^T(t)\mathbf{Q}\mathbf{e}_x(t)+\mathbf{e}_u^T(t)\mathbf{R}\mathbf{e}_u(t)\ dt$ 
%+ \mathbf{e}_x^T(t+N)\mathbf{S}\mathbf{e}_x(t+N)$
\& $\mathbf{u}\in\mathcal{U}$
%%%& t
& i
& p.c. (on)
& $t_H=0.4\si{s}$ / $N=40$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{ligthart2017experimentally}} 
& $\mathbf{x}=[\phi \, \theta \, \dot{\phi} \, \dot{\theta} \, \dot{\psi}]^{\top}$  
\& $\mathbf{u}=[{f}_i|_{i=1}^6]^{\top}$ %he is actualyy controlly only 3, the other 3 are symmetrical
& l
& exp  
& hexarotor
\\ 
%\cline{2-5}
&  $\sum_{i=1}^{N}\big(\mathbf{e}^T_{x,i}\mathbf{Q}\mathbf{e}_{x,i} + \mathbf{\Delta}^T_{u,i}\mathbf{R}_1\mathbf{\Delta}_{u,i} +\mathbf{e}^T_{u,i}\mathbf{R}_2\mathbf{e}_{u,i}\big)$
% + \mathbf{e}^T_{x,N}\mathbf{Q}\mathbf{e}_{x,N}$ 
\& unconstrained
%%%& t
& e
& a.c. (on)
& $t_H=4\si{s}$ / $N=500$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{lin2016model}} 
& $\mathbf{x}=[\phi \, \theta \, \psi \, \dot{\phi} \, \dot{\theta} \, \dot{\psi}]^{\top}$  
\& $\mathbf{u}=[{f}_i|_{i=1}^4]^{\top}$
& l
& sim  
& quadrotor
\\ 
%\cline{2-5}
&  $\sum_{i=1}^{N-1}\big(\mathbf{e}^T_{x,i}\mathbf{Q}\mathbf{e}_{x,i} + \mathbf{\Delta}^T_{u,i}\mathbf{R}\mathbf{\Delta}_{u,i}\big) + \mathbf{e}^T_{x,N}\mathbf{Q}\mathbf{e}_{x,N}$
\& $\mathbf{x}\in \mathcal{X},\mathbf{u}\in\mathcal{U}$
%%%& r
& i
& t.p. (off)
& $t_H=0.4\si{s}$ / $N=20$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{liu2012explicit}} 
& $\mathbf{x}=[\mathbf{p}_W^{\top} \, \dot{\mathbf{p}}_B^{\top} \, \boldsymbol{\Theta}^{\top} \,\boldsymbol{\omega}^{\top}]^{\top}$  
\& $\mathbf{u}=[\delta_{lat,lon,ped,col}]^{\top}$
& nl 
& sim / exp 
& helicopter
\\ 
%\cline{2-5}
&  $\frac{1}{2}\int_0^{T}\mathbf{e}_x^T(t+\tau)\mathbf{Q}\mathbf{e}_x(t+\tau)\ d\tau$
\& unconstrained
%%%& t
& e
& fs.c (on)
& $t_H=4\si{s}$ / $T_{\text{MPC}}=0.2\si{s}$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{liu2015robust}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \ddot{\mathbf{p}}^{\top}]^{\top}$  
\& $\mathbf{u}=[\dddot{\mathbf{p}}^{\top}]$
& l (ad)
& sim / exp 
& quadrotor
\\ 
%\cline{2-5}
&  $\sum_{k=1}^{N}\big(\mathbf{u}[k]^T\mathbf{P}\mathbf{u}[k]+\mathbf{e}_x[k]^T\mathbf{L}_s\mathbf{e}_x[k]\big)$ 
%+\mathbf{e}_x[N]^T\mathbf{L}_t\mathbf{e}_x[N]$ if you want to replace this, index of the sum up to N-1 
\& $\mathbf{x}\in \mathcal{X}, \mathbf{u}\in\mathcal{U}$
%%%& r / t
& i
& t.p. (on)
& $t_H=1\si{s}$ / $N=50$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{mueller2013model}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \ddot{\mathbf{p}}^{\top}]^{\top}$  
\& $\mathbf{u}=\dddot{\mathbf{p}}$
& l (ad)
& exp 
& quadrotor (+ racket)
\\ 
%\cline{2-5}
&  $ \int_0^T (\dddot{x}(t))^2_j dt,\ j=1,2,3$
\& $\mathbf{x}\in \mathcal{X},\mathbf{u}\in\mathcal{U}$
%(feasibility on $T,\boldsymbol{\omega}$ checked a posteriori)
%%%& r
& i
& t.p. (off)
& d.h. / $N$ from $10$ to $200$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{mueller2013computationally}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \dot{\mathbf{p}}^{\top} \, \ddot{\mathbf{p}}^{\top}]^{\top}$  
\& $\mathbf{u}=\dddot{\mathbf{p}}$
& l (ad)
& exp 
& quadrotor (+ racket)
\\ 
%\cline{2-5}
&  $ \int_0^T (\dddot{x}(t))^2_j dt,\ j=1,2,3$
\& unconstrained 
%(feasibility on $T,\boldsymbol{\omega}$ checked a posteriori)
%%%& r
& e
& t.p. (off)
& d.h. / $T_{\text{MPC}}=0.02\si{s}$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{neunert2016fast}} 
& $\mathbf{x}=[\mathbf{p}^{\top} \, \boldsymbol{\Theta}^{\top} \, \dot{\mathbf{p}}^{\top} \,\boldsymbol{\omega}^{\top}]^{\top}$  
\& $\mathbf{u}=[f_i|_{i=1}^6]^{\top}$
& nl
& exp 
& ballbot, hexarotor
\\ 
%\cline{2-5}
&  $\int_{t=0}^{t_f}\mathbf{e}_x^T(t)\mathbf{Q}\mathbf{e}_x(t)+\ \mathbf{u}_x^T(t)\mathbf{R}\mathbf{e}_u(t)+W(x,t)\ dt$
\& unconstrained 
%%%& r / t
& i
& fs.c. (on)
& d.h. / $T_{\text{MPC}}\le 25\si{ms}$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{papachristos2013model}} 
& $\mathbf{x}=[x \, \dot{x} \, y \, \dot{y} \, z \, \dot{z}]^{\top}$  
\& $\mathbf{u}=[\phi_r \, \gamma_x \, T_z]^{\top}$
& l (ad)
& exp 
& tri-tiltrotor
\\ 
%\cline{2-5}
& $\sum_{i=1}^{N_p} \tilde{\mathbf{e}}_{x,i}^T \mathbf{Q} \tilde{\mathbf{e}}_{x,i}
+ \sum_{i=1}^{N_c - 1} {\mathbf{\delta{u}}}_{i}^T \mathbf{R} {\mathbf{\delta{u}}}_{i}
+ \sum_{i=1}^{N_p} {\mathbf{e}}_{u,i}^T \mathbf{N} {\mathbf{e}}_{u,i}$
\& $\mathbf{u}\in\mathcal{U}$
%%%& t
& e
& p.c. (on)
& $t_H=0.8\si{s}$ / $N=8$
\\
\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{white}
\multirow{2}{2.5cm}{\citedb{papachristos2013hybrid}} 
& $\mathbf{x}=[\theta \, q \, u \, w \, \alpha]^{\top}$  
\& $\mathbf{u}=[\Omega_F \, \Omega_B \, \delta_{\alpha_F} \, \delta_{\alpha_B} \, \alpha_r]^{\top}$
& l
& sim 
& quad-tiltrotor
\\ 
%\cline{2-5}
& $\sum_{k=0}^{N-1} \big( \mathbf{e}_{x,k}^T \mathbf{Q} \mathbf{e}_{x,k} + \mathbf{u}_{k}^T \mathbf{R} \mathbf{u}_{k} \big) + \mathbf{e}_{x,N}^T \mathbf{P} \mathbf{e}_{x,N}$
\& $\mathbf{x}\in \mathcal{X}, \mathbf{u}\in\mathcal{U}$
%%%& t
& e
& ps.c. %(off)
& $t_H=0.04\si{s}$ / $N=4$
\\
\tabucline[1pt]{-}
%\tabucline[1pt on 3pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%chen2017 & \multicolumn{4}{c |[1pt]}{
%%%%%presentation of a fast NMPC strategy to reduce the online optimization cost and comparison to other techniques
%%%%%} 
%%%%%\\
%%%%%\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%diehl2005 & \multicolumn{4}{c |[1pt]}{
%%%%%survey of numerical approaches to solve nl problems + overview of algorithmic developments fore real-time NMPC
%%%%%} 
%%%%%\\
%%%%%\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%kamel2017b & \multicolumn{4}{c |[1pt]}{
%%%%%implementation of LMPC and NMPC (ROS) on a hexarotor \& fixed-wing, using methods proposed in [kamel2017]
%%%%%} 
%%%%%\\
%%%%%\tabucline[1pt]{-}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%mueller2015 & \multicolumn{4}{c |[1pt]}{
%%%%%journal paper extending the work in [Mueller2013] and [Mueller2013b], applied to a quadrotor catching a ball
%%%%%} 
%%%%%\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\tabucline[1pt]{-}
%
\end{tabu}

} %end resizebox
\end{table*}
%%%\end{center}
